$V_kD:$ Improving Knowledge Distillation using Orthogonal Projections

Knowledge distillation is an effective method for training small and efficient deep learning models. However, the efficacy of a single method can degenerate when transferring to other tasks, modalities, or even other architectures. To address this limitation, we propose a novel constrained feature distillation method. This method is derived from a small set of core principles, which results in two emerging components: an orthogonal projection and a task-specific normalisation. Equipped with both of these components, our transformer models can outperform all previous methods on ImageNet and reach up to a 4.4% relative improvement over the previous state-of-the-art methods. To further demonstrate the generality of our method, we apply it to object detection and image generation, whereby we obtain consistent and substantial performance improvements over state-of-the-art. Code and models are publicly available: https://github.com/roymiles/vkd

==> tables/ablation/projection.tex <==
\begin{tabular}{cccc}
    \toprule
    \belowrulesepcolor{mygrey} 
    Constraint. & Assumption. Acc@1 & Acc@5 \\
    \aboverulesepcolor{mygrey}
    \midrule
    Affine & \#1 & - & - \\  
    Somen & \#2 &  - & - \\   
    \rowcolor{myblue} Orthonormal & \#1, \#2 & - & - \\ 
    \aboverulesepcolor{myblue}
    \bottomrule
\end{tabular}

==> tables/rebuttal/density_coverage.tex <==
\begin{tabular}{lcccccc}
    \toprule
    \belowrulesepcolor{mygrey}
    \rowcolor{mygrey} & \multicolumn{2}{c}{CIFAR-10} & \multicolumn{2}{c}{CIFAR-100} \\ 
    \rowcolor{mygrey} \multirow{-2}{*}{Normalisation} & Density ($\uparrow$) & Coverage ($\uparrow$) & Density ($\uparrow$) & Coverage ($\uparrow$) \\
    \aboverulesepcolor{mygrey}
    \midrule
    Layer Norm & 1.07 & 0.95 & - & - \\
    \rowcolor{myblue} Whitening & \textbf{1.22} & \textbf{0.98} & - & - \\
    \aboverulesepcolor{myblue}
    \bottomrule
\end{tabular}
